LLM-Independent Adaptive RAG: Let the Question Speak for Itself

Large Language Models~(LLMs) are prone to hallucinations, and Retrieval-Augmented Generation (RAG) helps mitigate this, but at a high computational cost while risking misinformation. Adaptive retrieval aims to retrieve only when necessary, but existing approaches rely on LLM-based uncertainty estimation, which remain inefficient and impractical. In this study, we introduce lightweight LLM-independent adaptive retrieval methods based on external information. We investigated 27 features, organized into 7 groups, and their hybrid combinations. We evaluated these methods on 6 QA datasets, assessing the QA performance and efficiency. The results show that our approach matches the performance of complex LLM-based methods while achieving significant efficiency gains, demonstrating the potential of external information for adaptive retrieval.

==> tables/OOD.tex <==
\begin{table*}[ht!]
    \centering
    \small
    \resizebox{\textwidth}{!}{

    \begin{tabular}{lccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{{Method}} & \multicolumn{3}{c|}{NQ} & \multicolumn{3}{c|}{SQUAD} & \multicolumn{3}{c|}{TQA} & \multicolumn{3}{c|}{2Wiki} & \multicolumn{3}{c|}{HotPot} & \multicolumn{3}{c}{Musique} \\
    \cmidrule{2-19}
     % & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC \\
      & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ \\
    \midrule
    Never RAG & 0.446 & 1.0 & 0.00 & 0.176 & 1.0 & 0.00 & 0.636 & 1.0 & 0.00 & 0.318 & 1.0 & 0.00 & 0.286 & 1.0 & 0.00 & 0.106 & 1.0 & 0.00 \\

    Always RAG & 0.496 & 1.0 & 1.00 & 0.312 & 1.0 & 1.00 & 0.610 & 1.0 & 1.00 & 0.374 & 1.0 & 1.00 & 0.410 & 1.0 & 1.00 & 0.100 & 1.0 & 1.00 \\
    
    \midrule
    AdaptiveRAG & \textbf{0.496} & 2.0 & 0.98 & 0.286 & 2.0 & 0.97 & 0.636 & 1.5 & 0.54 & 0.454 & 5.2 & 2.64 & \textbf{0.44} & 4.7 & 2.41 & \textbf{0.154} & 3.6 & 3.63 \\
    DRAGIN & 0.480 & 4.5 & 2.24 & \textbf{0.298} & 4.3 & 2.14 & \textbf{0.667} & 4.0 & 2.0 & \textbf{0.456} & 5.8 & 2.92 & 0.435 & 5.1 & 2.5 & 0.134 & 6.3 & 3.15 \\
    FLARE & 0.462 & 4.26 & 2.0 & 0.288 & 3.2 & 2.5 & 0.648 & 2.1 & 1.39 & 0.424 & 3.9 & 2.85 & 0.372 & 5.1 & 4.07 & 0.106 & 4.3 & 3.11 \\
    Seakr & 0.406 & 14.6 & 1.00 & 0.286 & 14.0 & 1.00 & 0.656 & 14.6 & 1.00 & 0.398 & 12.3 & 2.44 & 0.424 & 9.9 & 1.76 & 0.118 & 12.3 & 2.40 \\


    \midrule
    Ideal & 0.608 & 1.6 & 0.55 & 0.360 & 1.8 & 0.82 & 0.736 & 1.4 & 0.36 & 0.500 & 1.7 & 0.68 & 0.460 & 1.7 & 0.71 & 0.164 & 1.9 & 0.89 \\

    \bottomrule
    \end{tabular}
    }

    \caption{QA Performance of adaptive retrieval fine-tuned with in-domain data. `Ideal' represents the performance of a system with an oracle providing ideal predictions for the need to retrieve. `InAcc' denotes In-Accuracy, measuring the QA system's performance. `LMC' indicates the mean number of LM calls per question, and `RC' represents the mean number of retrieval calls per question. AdaptiveRAG and DRAGIN methods show the best performance.}
    \label{tab:main_ID_results}

\end{table*}




% \begin{table*}[ht!]
%     \centering
%     \begin{tabular}{lcccccc}
%         \toprule
%         & nq & trivia & squad & hotpotqa & 2wiki & musique \\
%         \midrule
%         nq      & 0.406 & 0.618 & 0.286 & 0.432 & 0.398 & 0.112 \\
%         trivia  & 0.274 & 0.656 & 0.166 & 0.386 & 0.366 & 0.116 \\
%         squad   & 0.406 & 0.618 & 0.286 & 0.432 & 0.398 & 0.112 \\
%         hotpotqa & 0.406 & 0.618 & 0.286 & 0.432 & 0.398 & 0.112 \\
%         2wiki   & 0.406 & 0.618 & 0.286 & 0.436 & 0.398 & 0.118 \\
%         musique & 0.406 & 0.618 & 0.286 & 0.436 & 0.398 & 0.118 \\
%         \bottomrule
%     \end{tabular}
%     \caption{In-Acc Values for SeaKR (ID/OOD)}
%     \label{tab:seakr}

% \end{table*}

% \begin{table*}[ht!]
%     \centering
%     \begin{tabular}{lcccccc}
%         \toprule
%         & nq & trivia & squad & hotpotqa & 2wiki & musique \\
%         \midrule
%     nq & 0.480 & 0.620 & 0.284 & 0.435 & 0.463 & 0.126 \\
%     trivia & 0.447 & 0.667 & 0.256 & 0.346 & 0.414 & 0.107 \\
%     squad & 0.460 & 0.627 & 0.298 & 0.430 & 0.447 & 0.134 \\
%     hotpotqa & 0.480 & 0.617 & 0.291 & 0.435 & 0.316 & 0.123 \\
%     2wiki & 0.428 & 0.611 & 0.275 & 0.421 & 0.456 & 0.120 \\
%     musique & 0.460 & 0.627 & 0.298 & 0.430 & 0.447 & 0.134 \\
%     \bottomrule
%     \end{tabular}
%     \caption{In-Acc Values for DRAGIN (ID/OOD)}
%     \label{tab:seakr}

% \end{table*}

% \begin{table*}[ht!]
%     \centering
%     \begin{tabular}{lcccccc}
%         \toprule
%          & 2wiki & hotpotqa & musique & nq & squad & trivia \\
%         \midrule
%         2wiki & 0.424 & 0.293 & 0.106 & 0.433 & 0.277 & 0.605 \\
%         hotpotqa & 0.384 & 0.372 & 0.093 & 0.448 & 0.277 & 0.612 \\
%         musique & 0.424 & 0.293 & 0.106 & 0.433 & 0.277 & 0.605 \\
%         nq & 0.374 & 0.256 & 0.090 & 0.462 & 0.264 & 0.607 \\
%         squad & 0.375 & 0.276 & 0.087 & 0.447 & 0.288 & 0.626 \\
%         trivia & 0.367 & 0.285 & 0.083 & 0.441 & 0.283 & 0.648 \\
%         \bottomrule
%     \end{tabular}
%     \caption{In-Acc Values for FLARE (ID/OOD)}
%     \label{tab:seakr}

% \end{table*}

% \begin{table*}[ht!]
%     \centering
%     \begin{tabular}{lcccccc}
%         \midrule
%         nq       & 0.496 & 0.626 & 0.276 & 0.440 & 0.438 & 0.142 \\
%         trivia   & 0.490 & 0.636 & 0.286 & 0.438 & 0.440 & 0.139 \\
%         squad    & 0.490 & 0.636 & 0.286 & 0.438 & 0.440 & 0.146 \\
%         hotpotqa & 0.490 & 0.636 & 0.284 & 0.440 & 0.440 & 0.148 \\
%         2wiki    & 0.490 & 0.632 & 0.269 & 0.440 & 0.454 & 0.136 \\
%         musique  & 0.490 & 0.624 & 0.254 & 0.438 & 0.420 & 0.154 \\
%         \bottomrule
%     \end{tabular}
%     \caption{In-Acc Values for AdaptiveRAG (ID/OOD)}
%     \label{tab:seakr}

%\end{table*}

==> tables/UE_description_part1.tex <==
% \begin{table*}
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method\\ acronym\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method \\ full name\end{tabular}}}           & \multicolumn{1}{c}{\textbf{Category}}                        & \multicolumn{1}{c}{\textbf{Compute}} & \multicolumn{1}{c}{\textbf{Memory}} & \multicolumn{1}{c}{\textbf{Short description}}  
% \\ \midrule



% \begin{tabular}[c]{@{}l@{}}CCP  \\ \cite{DBLP:conf/acl/FadeevaRSPLMTKP24}\end{tabular}                                                                                  & \begin{tabular}[c]
% {@{}l@{}}Claim-\\ Conditioned\\ Probability\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}Meaning\\  diversity\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The method aggregates token-level uncertainties\\ into a claim-level score, it removes the impact of\\ uncertainty about what claim to generate on the\\ current step and what surface form to use. 
% \vspace{1.1ex}
% \end{tabular}                                                                                                                                                                                                                              \\
% \begin{tabular}[c]{@{}l@{}}DegMat  \\ \cite{lin2023generating}\end{tabular}                                                                                & \begin{tabular}[c]{@{}l@{}}Degree \\ matrix\end{tabular}                                           & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}Using the Degree matrix a new uncertainty measure\\ could be found that reflects the average pairwise\\ distance.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                \\
% \begin{tabular}[c]{@{}l@{}}Eccentricity  \\ \cite{lin2023generating}\end{tabular}                                                                            & Eccentricity                                                                                       & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The smallest k eigenvectors of Laplacian Graph are \\ used as the proxy for the models’ embeddings. Then, \\ we could use the average offset from the average \\ embedding as the uncertainty measure.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                \\
% \begin{tabular}[c]{@{}l@{}}EigValLaplacian \\ \cite{lin2023generating}\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}}Sum of \\ eigenvalues of \\ the graph \\ Laplacian\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The score uses pairwise similarities between the \\ sampled answers to the questions to form the \\ symmetric weighted adjacency matrix (degree matrix). \\ This matrix is further used to create the graph\\ Laplacian. The sum of Eigenvalues of the Graph\\ Laplacian are used as a measure of uncertainty.
% \vspace{1.1ex}

% \end{tabular}                                              


% \\
% \begin{tabular}[c]{@{}l@{}}FisherRao \\ \cite{DBLP:conf/emnlp/DarrinPC23}\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Fisher-Rao\\ distance\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}FisherRao is a distance on the Riemannian space \\ formed by the parametric distributions, using the\\ Fisher information mmatrix as its metric. It \\ computes the geodesic distance between two \\ discrete distributions.

% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                     \\
% \begin{tabular}[c]{@{}l@{}}Hybrid \\ \cite{DBLP:conf/acl/VazhentsevKTPPB23}\end{tabular}                                                                                 & \begin{tabular}[c]{@{}l@{}}Hybrid \\ Uncertainty\\ Quantification\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}Hybrid uncertainty estimation (UE) method that\\ combines epistemic (model) and aleatoric (data)\\ UE methods.

% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                   \\
% \begin{tabular}[c]{@{}l@{}}Lex-Similarity \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                     & \begin{tabular}[c]{@{}l@{}}Lexical \\ similarity\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Meaning\\ Diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The score computes how similar two words or\\ phrases are in terms of their meaning.

% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                             \\
% \begin{tabular}[c]{@{}l@{}}Max Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Maximum \\ Token \\ Entropy\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The maximum entropy of all\\ tokens in the generated sequence.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                                                   \\
% Max Probability                                                                       & \begin{tabular}[c]{@{}l@{}}Maximum\\ Sequence\\ Probability\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score leverages the probability of the most\\ likely sequence generation.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                 \\
% \begin{tabular}[c]{@{}l@{}}MD \\ \cite{DBLP:conf/nips/LeeLLS18}\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}Mahalanobis\\  distance\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}In this paper, the authors propose a simple yet\\ effective method for detecting any abnormal\\ samples, which is applicable to any pre-trained\\ softmax neural classifier. They obtain the class \\ conditional Gaussian distributions with respect to \\ (low- and upper-level) features of the deep models\\ under Gaussian discriminant analysis, which result\\ in a confidence score based on the Mahalanobis\\ distance.
% \vspace{1.1ex}

% \end{tabular} \\



% \begin{tabular}[c]{@{}l@{}}Mean CPMI \\ \cite{DBLP:conf/emnlp/PoelCM22}\end{tabular}                                                                             & \begin{tabular}[c]{@{}l@{}}Mean conditional\\ pointwise mutual\\  information\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Medium                               & Medium                              & \begin{tabular}[c]{@{}l@{}}Extension of the PMI method by considering only\\ those marginal probabilities for which the entropy\\ of the conditional distribution is above certain\\ threshold.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                             \\
% \begin{tabular}[c]{@{}l@{}}Mean Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Mean Token\\ Entropy\end{tabular}                                       & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The average entropy of each individual\\ token in the generated sequence.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                  \\
% \begin{tabular}[c]{@{}l@{}}Mean PMI \\ \cite{takayama2019relevant}\end{tabular}                                                                              & \begin{tabular}[c]{@{}l@{}}Mean pointwise\\ mutual information\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Medium                               & Low                                 & \begin{tabular}[c]{@{}l@{}}PMI compares the probability of two events (the \\ question and the generated answer) occurring together\\ to what this probability would be if the events were\\ independent.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                   \\
% Mean Probability                                                                      & \begin{tabular}[c]{@{}l@{}}Mean Sequence\\ Probability\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The total uncertainty is measured via average\\  sequence probability.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                                           \\
% \begin{tabular}[c]{@{}l@{}}Median Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                       & \begin{tabular}[c]{@{}l@{}}Median Token\\ Entropy\end{tabular}                                     & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The median entropy of all\\ tokens in the generated sequence.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                                                    \\
% Median Probability                                                                    & \begin{tabular}[c]{@{}l@{}}Median Sequence\\ Probability\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The total uncertainty is measured via \\ median sequence probability.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                                            \\
% \begin{tabular}[c]{@{}l@{}}Min Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                           & \begin{tabular}[c]{@{}l@{}}Minimum Token\\ Entropy\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The minimum entropy of all\\ tokens in the generated sequence.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                                                   \\
% Min Probability                                                                       & \begin{tabular}[c]{@{}l@{}}Minimum Sequence\\ Probability\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score leverages the probability of the least\\ likely sequence generation.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                                                                                                                                                                                                                                   \\ 
% \begin{tabular}[c]{@{}l@{}}NumSemSets   \\ \cite{lin2023generating}\end{tabular}  
% & \begin{tabular}[c]{@{}l@{}}Number of semantic\\ sets\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}Meaning \\ Diversity\end{tabular} & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The number of semantic sets initially equals the total\\ number of generated answers K. If two answers are \\ semantically similar, they are put into one cluster. \\ A higher number of semantic sets corresponds to an\\ increased level of uncertainty, as it suggests a higher\\ number of diverse semantic interpretations for the\\ answer.
% \vspace{1.1ex}

% \end{tabular}                                                                                                                                       \\
% \bottomrule
% % RDE                                                                                   & \begin{tabular}[c]{@{}l@{}}Robust density\\ estimation\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The method improves over MD by reducing\\  the dimensionality of the last hidden state of the\\ decoder averaged over all generated tokens via PCA\\ decomposition.  Additionally, computing of the  \\ covariance matrix for each individual class is done\\ by using the Minimum Covariance Determinant\\ estimation. The uncertainty score is computed as \\ the MD in the space of reduced dimensionality.\end{tabular}                   \\
% % RenyiNeg                                                                              & Rényi negentropy                                                                                   & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score computes alpha-Renyi-divergence \\ between the sample and the uniform distributions.\end{tabular}                                                                                                                                                                                                                                                                                                                                   \\
% % RMD                                                                                   & \begin{tabular}[c]{@{}l@{}}Relative\\ Mahalanobis\\ distance\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The MD distance score is adjusted by subtracting\\ from it the other  MD score computed for some\\ large general purpose dataset covering many\\ domains.\end{tabular}                                                                                                                                                                                                                                                                        \\
% % SAR                                                                                   & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}SAR corrects generative inequalities by reviewing\\ the relevance of each token and emphasizing\\ uncertainty quantification attention to those more\\ relevant components. The relevance is measured by\\ calculating similarity of sentence before and after\\ removing the certain token.\end{tabular}                                                                                                                                     \\
% % Semantic Entropy                                                                      & \begin{tabular}[c]{@{}l@{}}Semantic\\ Entropy\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The method aims to deal with the generated\\ sequences that have similar meaning while having\\ different probabilities according to the model. \\ The idea is to cluster generated sequences into several\\ semantically homogeneous clusters with a bi-directional\\ entailment algorithm and average the sequence\\ probabilities within the clusters.\end{tabular}                                                                        \\
% % SentenceSAR                                                                           & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant \\ at Sentence level\end{tabular} & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & SAR measured at sentence-level.                      
% \end{tabular}
% }
%     \label{tab:ue_desc1}
%     \caption{Description of the uncertainty features used in the paper.
%  }

% \end{table*}

\begin{table*}[ht!]
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\toprule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method\\ acronym\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method \\ full name\end{tabular}}}           & \multicolumn{1}{c}{\textbf{Short description}}                                                                                                                                                                                                                                                                                                                                                                                                              \\ \midrule
\multicolumn{3}{c}{\textbf{logit based}}                                                                                

\\ \midrule

\vspace{1.5ex} 


\begin{tabular}[c]{@{}l@{}}FisherRao \\ \cite{DBLP:conf/emnlp/DarrinPC23}\end{tabular}                                                                              & \begin{tabular}[c]{@{}l@{}}Fisher-Rao\\ distance\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}FisherRao is a distance on the Riemannian space formed by the parametric distributions, using the Fisher\\ information matrix as its metric. It computes the geodesic distance between two discrete distributions.

\vspace{1.1ex}

\end{tabular}                                                                                                                                                                                                  \\
\begin{tabular}[c]{@{}l@{}}Max Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                           & \begin{tabular}[c]{@{}l@{}}Maximum Token \\ Entropy\end{tabular}                                   & The maximum entropy of all tokens in the generated  sequence.                                                                  \\
Max Probability                                                                       & \begin{tabular}[c]{@{}l@{}}Maximum Sequence\\ Probability\end{tabular}                             & The score leverages the probability of the most likely sequence generation.                                                                                                                                                                                                                                                                                                                                                                                 \\
\begin{tabular}[c]{@{}l@{}}Mean CPMI \\ \cite{DBLP:conf/emnlp/PoelCM22}\end{tabular}                                                                             & \begin{tabular}[c]{@{}l@{}}Mean conditional\\ pointwise mutual\\ information\end{tabular}          & \begin{tabular}[c]{@{}l@{}}Extension of the PMI method by considering only those marginal probabilities for which the entropy of the\\ conditional distribution is above certain threshold.\end{tabular}                                                                                                                                                                                                                                                    \\
\begin{tabular}[c]{@{}l@{}}Mean Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Mean Token\\ Entropy\end{tabular}                                       & The average entropy of each individual token in the generated sequence.                                                                       \vspace{1.1ex} 

\\
\begin{tabular}[c]{@{}l@{}}Mean PMI \\ \cite{takayama2019relevant}\end{tabular}                                                                              & \begin{tabular}[c]{@{}l@{}}Mean pointwise\\ mutual information\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}PMI compares the probability of two events (the  question and the generated answer)  occurring together to what\\ this probability would be if the events were independent.\end{tabular}                                                                                                                                                                                                                                         \\
Mean Probability                                                                      & \begin{tabular}[c]{@{}l@{}}Mean Sequence\\ Probability\end{tabular}                                & The total uncertainty is measured via average sequence probability.                                                                                                                                                                                                                                                                                                                                                                                         \\
\begin{tabular}[c]{@{}l@{}}Median Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                        & \begin{tabular}[c]{@{}l@{}}Median Token\\ Entropy\end{tabular}                                     & The median entropy of all tokens in the generated sequence.                                                                                                                                                                                                                                                                                                                                                                                                 \\
Median Probability                                                                    & \begin{tabular}[c]{@{}l@{}}Median Sequence\\ Probability\end{tabular}                              & The total uncertainty is measured via  median sequence probability.                                                                                                                                                                                                                                                                                                                                                                                         \\
\begin{tabular}[c]{@{}l@{}}Min Entropy \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                           & \begin{tabular}[c]{@{}l@{}}Minimum Token\\ Entropy\end{tabular}                                    & The minimum entropy of all tokens in the generated sequence.                                                                                                                                                                                                                                                                                                                                                                                                \\
Min Probability                                                                       & \begin{tabular}[c]{@{}l@{}}Minimum Sequence\\ Probability\end{tabular}                             & The score leverages the probability of the least likely sequence generation.                                                                                                                                                                                                                                                                                                                                                                                \\
\begin{tabular}[c]{@{}l@{}}Perplexity \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                            & Perplexity                                                                                         & The score computes the average negative log probability of generated tokens, which is further exponentiated.                          
\vspace{1.1ex} 

\\
\begin{tabular}[c]{@{}l@{}}PTrue \\ \cite{kadavath2022language}\end{tabular}                                                                                & probability P(true)                                                                                & \begin{tabular}[c]{@{}l@{}}The method measures the uncertainty of the claim  by asking the LLM itself whether the generated claim is true or\\ not.  The confidence is the probability of thefirst generated token y1 being equal to “True”.\end{tabular}                                                            \vspace{1.1ex}                                                                                                                                         \\
\begin{tabular}[c]{@{}l@{}}RenyiNeg  \\ \cite{DBLP:conf/emnlp/DarrinPC23}\end{tabular}                                                                               & Rényi negentropy                                                                                   & The score computes alpha-Renyi-divergence between the sample and the uniform distributions.                                                                                 \vspace{1.1ex}                                                                                                \\
\begin{tabular}[c]{@{}l@{}}SAR\\  \cite{duan2023shifting}\end{tabular}                                                                                    & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}SAR corrects generative inequalities by reviewing the relevance of each token and emphasizing uncertainty\\ quantification attention to those more relevant components. The relevance is measured by calculating similarity\\ of sentence before and after removing the certain token.\end{tabular}                                                                                                                              \\
\begin{tabular}[c]{@{}l@{}}SentenceSAR\\  \cite{duan2023shifting}\end{tabular}                                                                           & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant \\ at Sentence level\end{tabular} & SAR measured at sentence-level.                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
\multicolumn{3}{c}{\textbf{consistency based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \midrule
\vspace{1.5ex} 

\begin{tabular}[c]{@{}l@{}}CCP  \\ \cite{DBLP:conf/acl/FadeevaRSPLMTKP24}\end{tabular}                                                                                  & \begin{tabular}[c]
{@{}l@{}}Claim-Conditioned\\ Probability\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}The method aggregates token-level uncertainties into a claim-level score, it removes the impact of uncertainty \\ about what claim to generate on the current step and what surface form to use. 

\vspace{1.1ex}

\end{tabular} \\

\begin{tabular}[c]{@{}l@{}}DegMat  \\ \cite{lin2023generating}\end{tabular}                                                                                 & \begin{tabular}[c]{@{}l@{}}Degree \\ matrix
\end{tabular}                                           & Using the Degree matrix a new uncertainty measure could be found that reflects the average pairwise distance.        \vspace{1.1ex} 

\\
\begin{tabular}[c]{@{}l@{}}Eccentricity  \\ \cite{lin2023generating}\end{tabular}                                                                           & Eccentricity                                                                                       & \begin{tabular}[c]{@{}l@{}}The smallest k eigenvectors of Laplacian Graph are used as the proxy for the models’ embeddings. Then, we could\\ use the average offset from the average embedding as the uncertainty measure.\end{tabular}                                                                          \vspace{1.1ex}                                                                                                                                             \\
\begin{tabular}[c]{@{}l@{}}EigValLaplacian \\ \cite{lin2023generating}\end{tabular}                                                                       & \begin{tabular}[c]{@{}l@{}}Sum of  eigenvalues of \\ the graph Laplacian\end{tabular}              & \begin{tabular}[c]{@{}l@{}}The score uses pairwise similarities between the sampled answers to the questions to form the symmetric weighted\\ adjacency matrix (degree matrix). This matrix is further used to create the graph Laplacian. The sum of Eigenvalues\\ of the Graph Laplacian are used as a measure of uncertainty.\end{tabular}                       \vspace{1.1ex} 

\\
\begin{tabular}[c]{@{}l@{}}Lex-Similarity \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                       & \begin{tabular}[c]{@{}l@{}}Lexical \\ similarity\end{tabular}                                      & The score computes how similar two words or phrases are in terms of their meaning.                                                                                                                                                                                                                                                                                                                                                                          \\
\begin{tabular}[c]{@{}l@{}}NumSemSets   \\ \cite{lin2023generating}\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}Number of semantic\\ sets\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}The number of semantic sets initially equals the total number of generated answers K. If two answers are\\ semantically similar, they are put into one cluster. A higher number of semantic sets corresponds to an increased\\ level of uncertainty, as it suggests a higher number of diverse semantic interpretations for the answer.
 \vspace{1.1ex} 
 
\end{tabular}                                                                             \\ 

\begin{tabular}[c]{@{}l@{}}Semantic Entropy \\  \cite{DBLP:conf/iclr/KuhnGF23}\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}}Semantic\\ Entropy\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}The method aims to deal with the generated sequences that have similar meaning while  having different  probabilities \\ according to the model. The idea is to cluster generated sequences into several semantically  homogeneous \\ clusters with a bi-directional entailment algorithm and average the sequence  probabilities within the clusters.\end{tabular} \\


\midrule
\multicolumn{3}{c}{\textbf{internal-based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \midrule
\vspace{1.5ex} 


\begin{tabular}[c]{@{}l@{}}MD \\ \cite{DBLP:conf/nips/LeeLLS18}\end{tabular}                                                                                   & 
 
\begin{tabular}[c]{@{}l@{}}Mahalanobis\\ distance\end{tabular}                                     & \begin{tabular}[c]{@{}l@{}}In this paper, the authors propose a simple yet effective method for detecting any abnormal samples, which is\\ applicable to any pre-trained softmax neural classifier. They obtain the class conditional Gaussian distributions\\ with respect to (low- and upper-level) features of the deep modelsunder Gaussian discriminant analysis, which\\ result in a confidence score based on the Mahalanobis distance.\end{tabular} 
\vspace{1.1ex} 
 
\\
\begin{tabular}[c]{@{}l@{}}RDE \\ \cite{DBLP:conf/acl/YooKJK22}\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}Robust density\\ estimation\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}The method improves over MD by reducing the dimensionality of the last hidden state of the decoder averaged\\ over all generated tokens via PCA decomposition.  Additionally, computing  of the covariance matrix for each\\ individual class is done by using the Minimum Covariance Determinant estimation. The uncertainty score is\\ computed as  the MD in the space of reduced dimensionality.
\vspace{1.1ex} 
 
\end{tabular}                \\
\begin{tabular}[c]{@{}l@{}}RMD  \\ \cite{DBLP:conf/iclr/0006LZKSLL23}\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}Relative Mahalanobis\\ distance\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}The MD distance score is adjusted by subtracting from it the other  MD score computed for some\\ large general purpose dataset covering many domains.
\vspace{1.1ex} 
 
 \end{tabular}                                                                                                                                                                                                                                                               \\  \midrule
\multicolumn{3}{c}{\textbf{blended approach}}                                                                   \\ \midrule

Hybrid                                                                                     & 
 Hybrid
                                   &
\begin{tabular}[c]{@{}l@{}} Our hybrid approach that uses all uncertainty features defined in the table.\end{tabular} 
\vspace{1.1ex} 
 
\\

\bottomrule

\end{tabular}

}
   
    \caption{Description of the uncertainty estimation methods used in the paper. The methods are grouped by their categories: logit based, consistency-based, internal-based and hybrid.
     \label{tab:ue_desc}
 }

\end{table*}

==> tables/UE_description_part2.tex <==
\begin{table*}
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method\\ acronym\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method \\ full name\end{tabular}}}           & \multicolumn{1}{c}{\textbf{Category}}                        & \multicolumn{1}{c}{\textbf{Compute}} & \multicolumn{1}{c}{\textbf{Memory}} & \multicolumn{1}{c}{\textbf{Short description}}  
\\ \midrule

                                      
\begin{tabular}[c]{@{}l@{}}Perplexity \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                            & Perplexity                                                                                         & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score computes the average negative log\\ probability of generated tokens, which is further\\ exponentiated.
\vspace{1.1ex}

\end{tabular}                                                                                                                                                                                                                                                                                                                \\
\begin{tabular}[c]{@{}l@{}}PTrue \\ \cite{kadavath2022language}\end{tabular}                                                                                 & probability P(true)                                                                                & Reflexive                                                    & Medium                               & Low                                 & \begin{tabular}[c]{@{}l@{}}The method measures the uncertainty of the claim \\ by asking the LLM itself whether the generated claim\\ is true or not. The confidence is the probability of the\\ first generated token y1 being equal to “True”.
\vspace{1.1ex}

\end{tabular}  

\\


\begin{tabular}[c]{@{}l@{}}RDE \\ \cite{DBLP:conf/acl/YooKJK22}\end{tabular}                                                                                     & \begin{tabular}[c]{@{}l@{}}Robust density\\ estimation\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The method improves over MD by reducing\\  the dimensionality of the last hidden state of the\\ decoder averaged over all generated tokens via PCA\\ decomposition.  Additionally, computing of the  \\ covariance matrix for each individual class is done\\ by using the Minimum Covariance Determinant\\ estimation. The uncertainty score is computed as \\ the MD in the space of reduced dimensionality.
\vspace{1.1ex}

\end{tabular}                   \\

\begin{tabular}[c]{@{}l@{}}RenyiNeg  \\ \cite{DBLP:conf/emnlp/DarrinPC23}\end{tabular}                                                                              & Rényi negentropy                                                                                   & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score computes alpha-Renyi-divergence \\ between the sample and the uniform distributions.
\vspace{1.1ex}

\end{tabular}                                                                                                                   \\
\begin{tabular}[c]{@{}l@{}}RMD  \\ \cite{DBLP:conf/iclr/0006LZKSLL23}\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Relative\\ Mahalanobis\\ distance\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The MD distance score is adjusted by subtracting\\ from it the other  MD score computed for some\\ large general purpose dataset covering many\\ domains.
\vspace{1.1ex}

\end{tabular}                                                                                                                                                                                                        \\
\begin{tabular}[c]{@{}l@{}}SAR\\  \cite{duan2023shifting}\end{tabular}                                                                                         & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}SAR corrects generative inequalities by reviewing\\ the relevance of each token and emphasizing\\ uncertainty quantification attention to those more\\ relevant components. The relevance is measured by\\ calculating similarity of sentence before and after\\ removing the certain token.
\vspace{1.1ex}

\end{tabular}                                                                                                                                     \\
\begin{tabular}[c]{@{}l@{}}Semantic Entropy \\  \cite{DBLP:conf/iclr/KuhnGF23}\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}}Semantic\\ Entropy\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The method aims to deal with the generated\\ sequences that have similar meaning while having\\ different probabilities according to the model. \\ The idea is to cluster generated sequences into several\\ semantically homogeneous clusters with a bi-directional\\ entailment algorithm and average the sequence\\ probabilities within the clusters.
\vspace{1.1ex}

\end{tabular}                                                                        \\
\begin{tabular}[c]{@{}l@{}}SentenceSAR\\  \cite{duan2023shifting}\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant \\ at Sentence level\end{tabular} & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & SAR measured at sentence-level.            
\\ \bottomrule

\end{tabular}

}
    \label{tab:ue_desc2}
    \caption{Description of the uncertainty features used in the paper.
 }

\end{table*}

==> tables/all_UC.tex <==
% % table in appendix for all UC methods
% % both main results and proxy metrics


\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{

\begin{tabular}{ccccc|cccc|cccc}
\toprule
\multirow{2}{*}{{Method}}  & \multicolumn{4}{c|}{NQ} & \multicolumn{4}{c|}{SQUAD} & \multicolumn{4}{c}{TQA} \\
 & EM & F1 & InAcc & RC & EM & F1 & InAcc & RC & EM & F1 & InAcc & RC \\
\midrule
CCP & 0.398 & 0.512 & 0.496 & 0.94 & 0.252 & 0.389 & 0.312 & 1.00 & \textbf{0.600} & \textbf{0.692} & \textbf{0.662} & 0.28 \\
DegMat & 0.394 & 0.514 & 0.496 & 0.97 & 0.252 & 0.389 & 0.312 & 1.00 & 0.598 & 0.684 & 0.644 & 0.29 \\
Eccentricity & 0.404 & 0.520 & 0.500 & 0.84 & 0.252 & 0.390 & 0.312 & 1.00 & 0.594 & 0.677 & 0.638 & 0.21 \\
EigValLaplacian & 0.406 & 0.532 & \textbf{0.512} & 0.81 & 0.254 & 0.391 & 0.314 & 1.00 & 0.594 & 0.682 & 0.640 & 0.26 \\
FisherRao & 0.390 & 0.506 & 0.498 & 0.88 & 0.252 & 0.389 & 0.312 & 1.00 & 0.598 & 0.688 & 0.654 & 0.11 \\
Hybrid & 0.410 & 0.534 & 0.504 & 0.65 & 0.254 & 0.393 & 0.314 & 0.99 & 0.594 & 0.689 & 0.654 & 0.32 \\
Lex-Similarity & 0.420 & \textbf{0.535} & \textbf{0.512} & 0.58 & 0.256 & \textbf{0.394} & \textbf{0.318} & 0.96 & \textbf{0.600} & 0.689 & 0.646 & 0.22 \\
MD & 0.398 & 0.511 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.598 & 0.681 & 0.642 & 0.05 \\
Max Entropy & \textbf{0.422} & \textbf{0.535} & 0.506 & 0.73 & 0.252 & 0.389 & 0.312 & 1.00 & 0.598 & 0.689 & 0.650 & 0.22 \\
Max Probability & 0.418 & 0.532 & 0.502 & 0.82 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.683 & 0.646 & 0.21 \\
Mean CPMI & 0.390 & 0.506 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.675 & 0.640 & 0.02 \\
Mean Entropy & 0.402 & 0.514 & 0.498 & 0.88 & 0.254 & 0.392 & 0.314 & 0.95 & 0.598 & 0.687 & 0.650 & 0.30 \\
Mean PMI & 0.390 & 0.506 & 0.496 & 1.00 & 0.254 & 0.389 & 0.312 & 1.00 & 0.596 & 0.683 & 0.640 & 0.02 \\
Mean Probability & 0.404 & 0.512 & 0.498 & 0.77 & 0.258 & \textbf{0.394} & \textbf{0.318} & 0.98 & 0.592 & 0.681 & 0.642 & 0.06 \\
Median Entropy & 0.412 & 0.519 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.596 & 0.682 & 0.644 & 0.15 \\
Median Probability & 0.408 & 0.512 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.680 & 0.644 & 0.26 \\
Min Entropy & 0.398 & 0.515 & 0.504 & 0.93 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.675 & 0.636 & 0.00 \\
Min Probability & 0.398 & 0.515 & 0.502 & 0.91 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.675 & 0.636 & 0.00 \\
NumSemSets & 0.406 & 0.521 & 0.502 & 0.83 & 0.252 & 0.389 & 0.312 & 1.00 & 0.590 & 0.680 & 0.638 & 0.28 \\
PTrue & 0.388 & 0.506 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.676 & 0.636 & 0.00 \\
Perplexity & 0.404 & 0.515 & 0.498 & 0.77 & 0.256 & 0.392 & 0.316 & 0.98 & 0.594 & 0.683 & 0.646 & 0.16 \\
RDE & 0.388 & 0.506 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.588 & 0.670 & 0.634 & 0.08 \\
RMD & 0.394 & 0.508 & 0.496 & 1.00 & 0.252 & 0.389 & 0.312 & 1.00 & 0.592 & 0.675 & 0.636 & 0.00 \\
RenyiNeg & 0.402 & 0.517 & 0.498 & 0.96 & 0.252 & 0.389 & 0.312 & 1.00 & 0.594 & 0.688 & 0.654 & 0.24 \\
SAR & 0.410 & 0.526 & 0.500 & 0.79 & 0.254 & 0.389 & 0.312 & 1.00 & 0.590 & 0.681 & 0.642 & 0.29 \\
Semantic Entropy & 0.406 & 0.521 & 0.504 & 0.83 & \textbf{0.260} & 0.393 & 0.316 & 0.92 & 0.596 & 0.685 & 0.640 & 0.24 \\
SentenceSAR & 0.410 & 0.521 & 0.500 & 0.73 & 0.254 & 0.391 & 0.314 & 0.99 & 0.596 & 0.685 & 0.644 & 0.24 \\
\bottomrule
\end{tabular}
    }
    \caption{Detailed QA performance results for uncertainty methods on one-hop datasets. `InAcc' denotes In-Accuracy, and `EM' stands for Exact Match. Higher values indicate better performance. Bold values highlight the best results. Standard deviations for InAcc, EM, and F1 are $\approx 0.02 \pm 0.003$, calculated using bootstrapping.}
    \label{tab:ue_result_one_hop}
\end{table*}



\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{tabular}{ccccc|cccc|cccc}
\toprule
\multirow{2}{*}{{Method}}  & \multicolumn{4}{c|}{2Wiki} & \multicolumn{4}{c|}{HotPot} & \multicolumn{4}{c}{Musique} \\
 & EM & F1 & InAcc & RC & EM & F1 & InAcc & RC & EM & F1 & InAcc & RC \\
\midrule
% Seakr & 0.382 & 0.460 & 0.398 & 2.44 & 0.400 & 0.523 & 0.424 & 1.76 & 0.112 & 0.215 & 0.118 & 2.40 \\
% AdaptiveRAG & 0.384 & 0.471 & 0.454 & 2.64 & 0.396 & 0.499 & 0.414 & 2.34 & 0.122 & 0.216 & 0.140 & 3.63 \\
% All Context & 0.302 & 0.396 & 0.374 & 1.00 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.167 & 0.100 & 1.00 \\
% DRAGIN & 0.406 & 0.480 & 0.456 & 2.92 & 0.398 & 0.506 & 0.430 & 2.56 & 0.116 & 0.207 & 0.134 & 3.15 \\

% FLARE & 0.358 & 0.451 & 0.424 & 2.85 & 0.298 & 0.391 & 0.372 & 4.07 & 0.076 & 0.161 & 0.090 & 3.10 \\
% FS-RAG & 0.348 & 0.431 & 0.388 & 3.76 & 0.376 & 0.503 & 0.422 & 3.70 & 0.088 & 0.187 & 0.100 & 3.35 \\
% IRCoT & 0.362 & 0.460 & 0.454 & 4.38 & 0.414 & 0.516 & 0.438 & 3.45 & 0.116 & 0.221 & 0.138 & 4.08 \\

% No Context & 0.302 & 0.371 & 0.318 & 0.00 & 0.280 & 0.372 & 0.286 & 0.00 & 0.100 & 0.193 & 0.106 & 0.00 \\


% Rowen_CL & 0.002 & 0.083 & 0.444 & 7.87 & 0.002 & 0.084 & 0.354 & 7.67 & 0.002 & 0.034 & 0.104 & 9.52 \\
% Rowen_CM & 0.002 & 0.083 & 0.444 & 7.87 & 0.002 & 0.084 & 0.354 & 7.70 & 0.002 & 0.034 & 0.104 & 9.52 \\
% Rowen_Hybrid & 0.002 & 0.083 & 0.444 & 7.85 & 0.004 & 0.086 & 0.354 & 7.63 & 0.002 & 0.034 & 0.102 & 9.48 \\

% \midrule
CCP & 0.310 & 0.398 & 0.376 & 0.98 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.167 & 0.100 & 1.00 \\
DegMat & \textbf{0.314} & \textbf{0.407} & 0.382 & 0.95 & 0.386 & 0.498 & 0.410 & 1.00 & 0.088 & 0.168 & 0.100 & 1.00 \\
Eccentricity & 0.312 & 0.406 & \textbf{0.384} & 0.93 & \textbf{0.390} & \textbf{0.502} & \textbf{0.414} & 0.93 & 0.088 & 0.167 & 0.100 & 1.00 \\
EigValLaplacian & 0.312 & 0.405 & \textbf{0.384} & 0.98 & 0.384 & 0.501 & 0.410 & 0.91 & 0.088 & 0.169 & 0.102 & 1.00 \\
FisherRao & 0.306 & 0.399 & 0.378 & 0.98 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.169 & 0.100 & 1.00 \\
Hybrid & 0.298 & 0.391 & 0.368 & 0.93 & 0.384 & 0.491 & 0.406 & 0.94 & 0.090 & 0.169 & 0.102 & 1.00 \\
Lex-Similarity & 0.306 & 0.400 & 0.376 & 0.97 & 0.386 & 0.498 & 0.410 & 0.95 & 0.088 & 0.168 & 0.100 & 1.00 \\
MD & 0.302 & 0.397 & 0.374 & 1.00 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.167 & 0.100 & 1.00 \\
Max Entropy & 0.304 & 0.398 & 0.376 & 0.95 & \textbf{0.390} & 0.501 & \textbf{0.414} & 0.99 & 0.088 & 0.167 & 0.100 & 1.00 \\
Max Probability & 0.304 & 0.396 & 0.374 & 1.00 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.167 & 0.100 & 1.00 \\
Mean CPMI & 0.302 & 0.397 & 0.376 & 0.98 & 0.386 & 0.497 & 0.410 & 1.00 & 0.090 & 0.169 & 0.102 & 0.99 \\
Mean Entropy & 0.306 & 0.400 & 0.378 & 0.93 & 0.386 & 0.497 & 0.410 & 0.99 & 0.088 & 0.167 & 0.100 & 1.00 \\
Mean PMI & 0.310 & 0.399 & 0.382 & 0.96 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.167 & 0.100 & 1.00 \\
Mean Probability & 0.308 & 0.400 & 0.380 & 0.96 & 0.388 & 0.498 & 0.412 & 0.97 & \textbf{0.092} & \textbf{0.173} & \textbf{0.104} & 0.97 \\
Median Entropy & 0.308 & 0.398 & 0.378 & 0.98 & 0.386 & 0.497 & 0.410 & 1.00 & 0.088 & 0.167 & 0.100 & 1.00 \\
Median Probability & 0.304 & 0.397 & 0.376 & 0.94 & 0.386 & 0.497 & 0.410 & 1.00 & 0.090 & 0.169 & 0.102 & 1.00 \\
Min Entropy & 0.308 & 0.397 & 0.376 & 0.93 & 0.386 & 0.497 & 0.410 & 1.00 & 0.090 & 0.171 & \textbf{0.104} & 0.99 \\
Min Probability & 0.312 & 0.401 & 0.376 & 0.95 & 0.386 & 0.497 & 0.410 & 1.00 & 0.090 & 0.169 & 0.102 & 0.99 \\
NumSemSets & 0.304 & 0.396 & 0.374 & 1.00 & 0.386 & \textbf{0.502} & 0.412 & 0.95 & 0.088 & 0.167 & 0.100 & 1.00 \\
PTrue & 0.308 & 0.398 & 0.372 & 0.87 & 0.386 & 0.497 & 0.410 & 1.00 & 0.090 & 0.169 & 0.102 & 0.99 \\
Perplexity & 0.304 & 0.398 & 0.376 & 0.96 & 0.386 & 0.498 & 0.410 & 1.00 & 0.088 & 0.168 & 0.100 & 1.00 \\
RDE & 0.304 & 0.398 & 0.376 & 0.99 & 0.386 & 0.497 & 0.410 & 1.00 & 0.090 & 0.171 & 0.102 & 0.99 \\
RMD & 0.304 & 0.398 & 0.372 & 0.97 & 0.388 & 0.499 & 0.412 & 0.95 & 0.088 & 0.167 & 0.100 & 1.00 \\
RenyiNeg & 0.302 & 0.396 & 0.374 & 1.00 & \textbf{0.390} & 0.500 & \textbf{0.414} & 0.97 & 0.088 & 0.167 & 0.100 & 1.00 \\
SAR & 0.310 & 0.404 & 0.380 & 0.97 & 0.386 & 0.500 & 0.412 & 0.90 & 0.088 & 0.167 & 0.100 & 1.00 \\
Semantic Entropy & 0.304 & 0.398 & 0.374 & 1.00 & 0.386 & 0.499 & 0.412 & 0.93 & 0.088 & 0.169 & 0.102 & 1.00 \\
SentenceSAR & 0.308 & 0.403 & 0.376 & 0.89 & 0.384 & 0.498 & 0.410 & 0.90 & 0.088 & 0.167 & 0.100 & 1.00 \\

\bottomrule
\end{tabular}
}
    \caption{Detailed QA performance results for uncertainty methods on one-hop datasets. `InAcc' denotes In-Accuracy, and `EM' stands for Exact Match. Higher values indicate better performance. Bold values highlight the best results. Standard deviations for InAcc, EM, and F1 are $\approx 0.02 \pm 0.002$ for HotPotQA and 2Wiki and $\approx 0.01 \pm 0.001$ for Musique, calculated using bootstrapping.
    }
    \label{tab:ue_result_multi_hop}
\end{table*}


==> tables/all_baselines.tex <==

\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{tabular}{lccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{5}{c|}{NQ} & \multicolumn{5}{c|}{SQUAD} & \multicolumn{5}{c}{TQA} \\
 & EM & F1 & Acc & LLMC & RC & EM & F1 & Acc & LLMC & RC & EM & F1 & Acc & LLMC & RC \\
\midrule
No Context & 0.386 & 0.495 & 0.446 & 1.0 & 0.00 & 0.156 & 0.249 & 0.176 & 1.0 & 0.00 & 0.592 & 0.675 & 0.636 & 1.0 & 0.00 \\
All Context & 0.388 & 0.506 & 0.496 & 1.0 & 1.00 & 0.252 & 0.389 & 0.312 & 1.0 & 1.00 & 0.522 & 0.636 & 0.610 & 1.0 & 1.00 \\
\midrule
AdaptiveRAG & 0.388 & 0.505 & 0.496 & 1.0 & 0.98 & 0.238 & 0.366 & 0.286 & 1.0 & 0.97 & 0.564 & 0.656 & 0.628 & 0.5 & 0.54 \\

DRAGIN & 0.396 & 0.510 & 0.480 & 4.5 & 2.24 & 0.244 & 0.371 & 0.298 & 4.3 & 2.14 & 0.584 & 0.691 & 0.666 & 4.1 & 2.06 \\
FLARE & 0.358 & 0.477 & 0.450 & 3.1 & 2.07 & 0.190 & 0.303 & 0.238 & 3.1 & 2.08 & 0.570 & 0.674 & 0.648 & 2.1 & 1.39 \\
FS-RAG & 0.348 & 0.483 & 0.428 & 2.7 & 2.70 & 0.226 & 0.361 & 0.286 & 2.8 & 2.78 & 0.540 & 0.640 & 0.632 & 2.5 & 2.47 \\
IRCoT & 0.392 & 0.502 & 0.478 & 2.7 & 2.70 & 0.210 & 0.341 & 0.268 & 2.7 & 2.68 & 0.526 & 0.634 & 0.608 & 2.7 & 2.74 \\

Rowen\textsubscript{CL} & 0.002 & 0.104 & 0.494 & 29.5 & 7.24 & 0.004 & 0.061 & 0.196 & 29.2 & 7.19 & 0.022 & 0.188 & 0.656 & 28.7 & 7.06 \\
Rowen\textsubscript{CM} & 0.002 & 0.104 & 0.494 & 29.5 & 7.27 & 0.004 & 0.061 & 0.196 & 29.2 & 7.20 & 0.022 & 0.188 & 0.656 & 28.7 & 7.12 \\
Rowen\textsubscript{Hybrid} & 0.002 & 0.104 & 0.494 & 55.0 & 7.27 & 0.004 & 0.061 & 0.196 & 54.3 & 7.15 & 0.022 & 0.189 & 0.656 & 53.4 & 6.93 \\
Seakr & 0.360 & 0.487 & 0.406 & 14.6 & 1.00 & 0.226 & 0.361 & 0.268 & 14.6 & 1.00 & 0.598 & 0.692 & 0.656 & 14.6 & 1.00 \\
\bottomrule
\end{tabular}
}
    \caption{Results of baselines for onehop datasets. LLMC refers to the average number of LLM calls per question, while RC indicates the average number of retrieval calls per question. For NQ the standard deviations of Acc, EM, and F1 are $\approx 0.022 \pm 0.001$ across all methods.  For SQUAD and Trivia the standard deviations of Acc, EM, and F1 are $\approx 0.018 \pm 0.006$ across all methods.
    Overall, the methods exhibit similar deviations, with Rowen showing the lowest deviation, typically $\leq 0.01$.
    }
    \label{tab:one_hop_baseline}
\end{table*}

\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{tabular}{lccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{5}{c|}{2Wiki} & \multicolumn{5}{c|}{HotPotQA} & \multicolumn{5}{c}{Musique} \\
 & EM & F1 & Acc & LLMC & RC & EM & F1 & Acc & LLMC & RC & EM & F1 & Acc & LLMC & RC \\
\midrule
No Context & 0.302 & 0.371 & 0.318 & 1.0 & 0.00 & 0.280 & 0.372 & 0.286 & 1.0 & 0.00 & 0.100 & 0.193 & 0.106 & 1.0 & 0.00 \\
All Context & 0.302 & 0.396 & 0.374 & 1.0 & 1.00 & 0.386 & 0.497 & 0.410 & 1.0 & 1.00 & 0.088 & 0.167 & 0.100 & 1.0 & 1.00 \\
\midrule
AdaptiveRAG & 0.384 & 0.471 & 0.454 & 2.6 & 2.64 & 0.396 & 0.499 & 0.414 & 2.3 & 2.34 & 0.122 & 0.216 & 0.140 & 3.6 & 3.63 \\
DRAGIN & 0.406 & 0.480 & 0.456 & 5.8 & 2.92 & 0.398 & 0.506 & 0.430 & 5.1 & 2.56 & 0.116 & 0.207 & 0.134 & 6.3 & 3.15 \\
FLARE & 0.358 & 0.451 & 0.424 & 3.9 & 2.85 & 0.298 & 0.391 & 0.372 & 5.1 & 4.07 & 0.076 & 0.161 & 0.090 & 4.1 & 3.10 \\
FS-RAG & 0.348 & 0.431 & 0.388 & 3.8 & 3.76 & 0.376 & 0.503 & 0.422 & 3.7 & 3.70 & 0.088 & 0.187 & 0.100 & 3.4 & 3.35 \\
IRCoT & 0.362 & 0.460 & 0.454 & 4.4 & 4.38 & 0.414 & 0.516 & 0.438 & 3.5 & 3.45 & 0.116 & 0.221 & 0.138 & 4.1 & 4.08 \\
Rowen\textsubscript{CL} & 0.002 & 0.083 & 0.444 & 32.9 & 7.87 & 0.002 & 0.084 & 0.354 & 31.9 & 7.67 & 0.002 & 0.034 & 0.104 & 42.1 & 9.52 \\
Rowen\textsubscript{CM} & 0.002 & 0.083 & 0.444 & 32.9 & 7.87 & 0.002 & 0.084 & 0.356 & 31.9 & 7.70 & 0.002 & 0.034 & 0.104 & 42.1 & 9.52 \\
Rowen\textsubscript{Hybrid} & 0.002 & 0.083 & 0.444 & 61.8 & 7.85 & 0.004 & 0.086 & 0.354 & 59.8 & 7.63 & 0.002 & 0.034 & 0.102 & 80.2 & 9.48 \\
Seakr & 0.382 & 0.460 & 0.398 & 12.3 & 2.44 & 0.400 & 0.523 & 0.424 & 9.9 & 1.76 & 0.112 & 0.215 & 0.118 & 12.3 & 2.40 \\
\bottomrule
\end{tabular}
}
    \caption{Results of baselines for multihop datasets. LLMC refers to the average number of LLM calls per question, while RC indicates the average number of retrieval calls per question. For 2Wiki and HotPotQA, the standard deviations of Acc, EM, and F1 are $\leq 0.022 \pm 0.001$ across all methods. For Musique, the standard deviations are $\leq 0.015 \pm 0.001$. Overall, the methods exhibit similar deviations, with Rowen showing the lowest deviation, typically $\leq 0.01$.
    }
    \label{tab:multi_hop_baseline}
\end{table*}


==> tables/all_methods_mean_transfer_loss.tex <==
% show all methods mean transfer loss (average over datasets over all combinations)
% add significance tests over each pair to show dominance. 36 values is enough for ranked tests

\begin{table*}[t]
    \centering
    \begin{tabular}{lcccccc|c}
    \toprule
     & NQ & SQUAD & TQA & 2Wiki & HotPot & Musique & Avg \\
    \midrule
    Mean CPMI & -2.02 & -7.44 & -4.38 & -2.98 & -5.76 & 0.78 & -3.63 \\
    Mean PMI & -1.45 & -8.21 & -4.69 & -4.19 & -5.37 & 3.20 & -3.45 \\
    RDE & -1.29 & -7.18 & -3.52 & -2.23 & -4.68 & 1.18 & -2.95 \\
    PTrue & -1.94 & -7.95 & -3.77 & -2.03 & -5.07 & 3.53 & -2.87 \\
    EigValLaplacian & -3.28 & -7.01 & -3.44 & -2.29 & -3.32 & 2.35 & -2.83 \\
    Min Probability & -1.83 & -5.26 & -3.52 & -2.98 & -3.22 & 1.96 & -2.48 \\
    RenyiNeg & -1.04 & -4.23 & -6.12 & 0.21 & -3.38 & 2.40 & -2.03 \\
    NumSemSets & -0.96 & -5.90 & -3.39 & -0.21 & -3.20 & 1.60 & -2.01 \\
    FisherRao & -0.80 & -5.26 & -3.44 & -2.75 & -3.12 & 3.60 & -1.96 \\
    Min Entropy & -2.22 & -4.23 & -3.08 & -0.85 & -1.17 & 0.38 & -1.86 \\
    Median Entropy & -0.89 & -3.97 & -3.81 & -1.48 & -3.80 & 3.60 & -1.72 \\
    Median Probability & -1.13 & -2.44 & -4.60 & -0.11 & -3.41 & 1.96 & -1.62 \\
    Hybrid & -1.83 & -4.71 & -4.28 & -0.32 & -5.12 & 7.06 & -1.53 \\
    Mean Probability & -0.16 & -2.39 & -4.22 & -0.42 & -2.43 & 1.54 & -1.35 \\
    Max Entropy & -1.90 & -2.56 & -4.80 & -0.43 & -3.00 & 6.40 & -1.05 \\
    CCP & 0.32 & -2.18 & -6.77 & -0.64 & -2.44 & 6.00 & -0.95 \\
    Max Probability & -0.64 & -2.95 & -4.41 & -0.64 & -2.24 & 5.20 & -0.95 \\
    DegMat & 0.56 & -2.69 & -3.91 & -1.57 & -2.15 & 4.80 & -0.83 \\
    Lex-Similarity & -2.50 & -3.77 & -3.41 & -0.85 & -2.34 & 8.00 & -0.81 \\
    Eccentricity & 0.00 & -2.31 & -2.63 & -2.60 & -2.71 & 5.60 & -0.78 \\
    SAR & -0.24 & -2.31 & -2.87 & -1.05 & -3.11 & 5.60 & -0.66 \\
    SentenceSAR & 0.32 & -2.42 & -3.35 & -0.85 & -2.15 & 5.20 & -0.54 \\
    Semantic Entropy & -0.48 & -1.77 & -2.69 & 0.43 & -1.94 & 3.53 & -0.49 \\
    RMD & 0.08 & -7.56 & -1.76 & -0.11 & -0.49 & 7.60 & -0.37 \\
    Perplexity & 0.24 & -2.66 & -4.27 & 0.85 & -1.56 & 5.60 & -0.30 \\
    Mean Entropy & -0.48 & -1.40 & -3.94 & 0.74 & -1.76 & 7.20 & 0.06 \\
    MD & 0.00 & -2.56 & -2.74 & 0.65 & 0.00 & 9.60 & 0.82 \\
    \bottomrule
    \end{tabular}
    \caption{Average QA performance differences after transfer (in percentage) for each dataset. Negative values indicate a loss in In-Accuracy compared to in-domain testing, while positive values represent an In-Accuracy gain.}
    \label{tab:qa_transfer}
\end{table*}




==> tables/classifier_stability.tex <==
% table with how feature is stable over max - mean over different classifiers. will show the disentanglement (maybe)
% maybe changed or added with a figure

\begin{table*}[t]
    \centering
    \small
    %\resizebox{0.\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Method & Mean & Max & Difference \\
\midrule
Hybrid & 25.67 & 11.33 & -14.33 \\
RMD & 23.50 & 15.00 & -8.50 \\
Perplexity & 15.00 & 8.83 & -6.17 \\
MD & 19.50 & 13.50 & -6.00 \\
CCP & 15.50 & 9.67 & -5.83 \\
EigValLaplacian & 11.67 & 6.00 & -5.67 \\
Median Entropy & 15.67 & 10.67 & -5.00 \\
Mean Entropy & 12.83 & 8.33 & -4.50 \\
RDE & 16.83 & 12.67 & -4.17 \\
DegMat & 13.67 & 10.00 & -3.67 \\
Max Entropy & 10.00 & 6.50 & -3.50 \\
Mean CPMI & 14.00 & 11.00 & -3.00 \\
Lex-Similarity & 9.33 & 6.50 & -2.83 \\
SentenceSAR & 12.00 & 9.17 & -2.83 \\
Min Entropy & 11.83 & 9.33 & -2.50 \\
SAR & 10.50 & 8.83 & -1.67 \\
PTrue & 16.00 & 14.50 & -1.50 \\
Max Probability & 11.33 & 10.50 & -0.83 \\
Min Probability & 11.00 & 10.17 & -0.83 \\
FisherRao & 9.17 & 8.50 & -0.67 \\
Semantic Entropy & 9.17 & 8.50 & -0.67 \\
RenyiNeg & 9.00 & 9.33 & 0.33 \\
Mean Probability & 5.83 & 6.33 & 0.50 \\
Mean PMI & 10.33 & 11.17 & 0.83 \\
Median Probability & 8.83 & 9.83 & 1.00 \\
Eccentricity & 7.83 & 8.83 & 1.00 \\
NumSemSets & 10.33 & 12.00 & 1.67 \\
\bottomrule
\end{tabular}
%}
   \caption{Rank of UC methods by In-Accuracy, aggregated using the mean or maximum across different classifiers. A lower difference indicates reduced stability to classifier choice, whereas a higher difference reflects greater robustness to classifier choice.
}
    \label{tab:classifier_sens}
\end{table*}


% maybe add figure with top 3 UC distributions overlapped 

==> tables/main_2hop_proxy_metrics.tex <==
% table with proxy metrics for baselines, 3 top UC, Best UC
% Correlation, ROC-AUC, Overconfidence, Undercondifence, etc from ACL paper
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{

\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{3}{c}{2Wiki} & \multicolumn{3}{c}{HotPot} & \multicolumn{3}{c}{Musique} \\
 & Acc & Corr & AUC & Acc & Corr & AUC & Acc & Corr & AUC \\
\midrule
AdaptiveRAG & \textbf{0.724} & \textbf{0.339} & \textbf{0.710} & 0.708 & 0.189 & 0.621 & 0.876 & 0.149 & 0.640 \\
DRAGIN & 0.682 & -0.071 & 0.456 & 0.714 & 0.011 & 0.507 & 0.894 & -0.014 & 0.487 \\
FLARE & 0.514 & 0.200 & 0.623 & 0.418 & 0.059 & 0.537 & 0.592 & 0.011 & 0.511 \\
Rowen\textsubscript{CL} & 0.316 & -0.101 & 0.459 & 0.288 & -0.134 & 0.441 & 0.108 & 0.004 & 0.503 \\
Rowen\textsubscript{CM} & 0.318 & 0.018 & 0.508 & 0.290 & -0.143 & 0.440 & 0.110 & -0.019 & 0.487 \\
Rowen\textsubscript{Hybrid} & 0.316 & -0.036 & 0.482 & 0.292 & -0.168 & 0.412 & 0.108 & -0.010 & 0.492 \\
Seakr & 0.682 & -0.217 & 0.365 & 0.714 & 0.075 & 0.548 & 0.894 & 0.065 & 0.561 \\
\midrule
EigValLaplacian & 0.688 & 0.194 & 0.620 & 0.728 & 0.266 & 0.670 & 0.894 & 0.125 & 0.617 \\
Lex-Similarity & 0.684 & 0.215 & 0.634 & \textbf{0.728} & 0.297 & {0.690} & \textbf{0.896} & 0.084 & 0.594 \\
Max Entropy & 0.688 & 0.194 & 0.621 & 0.726 & 0.295 & 0.688 & 0.894 & \textbf{0.180} & \textbf{0.669} \\
SAR & 0.686 & 0.234 & 0.645 & \textbf{0.734} & 0.303 & 0.694 & 0.894 & 0.166 & 0.660 \\
Mean Entropy & 0.684 & 0.282 & 0.675 & 0.722 & \textbf{0.310} & \textbf{0.698} & \textbf{0.896} & 0.147 & 0.637 \\

\bottomrule
\end{tabular}


}

    \caption{Caption}
    \label{tab:multi_hop_proxy}
\end{table*}


==> tables/main_confidence.tex <==

\begin{table*}[th!]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{SQUAD} & \multicolumn{2}{c}{TQA} & \multicolumn{2}{c}{2Wiki} & \multicolumn{2}{c}{HotPot} & \multicolumn{2}{c}{Musique} \\
 & Over & Under & Over & Under & Over & Under & Over & Under & Over & Under & Over & Under \\
\midrule
AdaptiveRAG & 0.01 & 0.43 & 0.14 & 0.13 & 0.19 & 0.30 & 0.12 & 0.15 & 0.11 & 0.18 & 0.02 & 0.10 \\
DRAGIN & 0.00 & 0.45 & 0.00 & 0.18 & 0.00 & 0.64 & 0.00 & 0.32 & 0.00 & 0.29 & 0.00 & 0.11 \\

FLARE & 0.20 & 0.21 & 0.40 & 0.06 & 0.18 & 0.24 & 0.43 & 0.06 & 0.53 & 0.05 & 0.34 & 0.06 \\

Rowen\textsubscript{CL} & 0.55 & 0.00 & 0.82 & 0.00 & 0.36 & 0.00 & 0.68 & 0.00 & 0.71 & 0.00 & 0.89 & 0.00 \\
Rowen\textsubscript{CM} & 0.55 & 0.00 & 0.82 & 0.00 & 0.36 & 0.00 & 0.68 & 0.00 & 0.71 & 0.00 & 0.89 & 0.00 \\
Rowen\textsubscript{Hybrid} & 0.55 & 0.00 & 0.82 & 0.00 & 0.36 & 0.01 & 0.68 & 0.00 & 0.71 & 0.00 & 0.89 & 0.00 \\

Seakr & 0.00 & 0.45 & 0.00 & 0.18 & 0.00 & 0.64 & 0.00 & 0.32 & 0.00 & 0.29 & 0.00 & 0.11 \\
\midrule
Lex-Similarity & 0.01 & 0.21 & 0.00 & 0.15 & 0.18 & 0.06 & 0.00 & 0.28 & 0.02 & 0.22 & 0.00 & 0.10 \\
Max Entropy & 0.08 & 0.20 & 0.00 & 0.13 & 0.17 & 0.07 & 0.00 & 0.29 & 0.00 & 0.23 & 0.00 & 0.10 \\
EigValLaplacian & 0.03 & 0.33 & 0.00 & 0.17 & 0.21 & 0.08 & 0.00 & 0.30 & 0.01 & 0.23 & 0.00 & 0.10 \\
SAR & 0.06 & 0.29 & 0.00 & 0.16 & 0.18 & 0.09 & 0.00 & 0.28 & 0.03 & 0.22 & 0.00 & 0.11 \\
Mean Entropy & 0.04 & 0.29 & 0.00 & 0.14 & 0.14 & 0.07 & 0.00 & 0.29 & 0.00 & 0.15 & 0.00 & 0.10 \\
\bottomrule
\end{tabular}

}

    \caption{Over- and UnderConfidence for adaptive retrieval methods and uncertainty estimation. Values closest to zero indicate the best performance. UnderConfidence refers to cases where the method failed to detect self-knowledge despite its presence, while OverConfidence reflects cases where the method incorrectly detected self-knowledge when it was absent.}
    \label{tab:confidence}
\end{table*}


==> tables/main_proxy_metrics.tex <==
% table with proxy metrics for baselines, 3 top UC, Best UC
% Correlation, ROC-AUC, Overconfidence, Undercondifence, etc from ACL paper
% \begin{table*}[t]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{

% \begin{tabular}{lccccccccc}
% \toprule
% \multirow{2}{*}{{Method}} & \multicolumn{3}{c}{NQ} & \multicolumn{3}{c}{SQUAD} & \multicolumn{3}{c}{TQA} \\
%  & Acc & Corr & ROCAUC & Acc & Corr & ROCAUC & Acc & Corr & ROCAUC \\
% \midrule
% AdaptiveRAG & 0.566 & 0.061 & 0.535 & 0.728 & 0.101 & 0.577 & 0.508 & -0.023 & 0.486 \\
% DRAGIN & 0.554 & 0.122 & 0.571 & 0.824 & 0.105 & 0.580 & 0.364 & 0.034 & 0.520 \\
% FLARE & 0.586 & 0.161 & 0.594 & 0.540 & 0.110 & 0.583 & 0.582 & 0.122 & 0.573 \\
% Rowen\textsubscript{CL} & 0.448 & -0.144 & 0.436 & 0.176 & -0.061 & 0.468 & 0.636 & -0.069 & 0.465 \\
% Rowen\textsubscript{CM} & 0.448 & -0.033 & 0.486 & 0.176 & -0.055 & 0.471 & 0.636 & -0.126 & 0.441 \\
% Rowen\textsubscript{Hybrid} & 0.448 & -0.121 & 0.438 & 0.174 & -0.070 & 0.456 & 0.626 & -0.125 & 0.431 \\
% Seakr & 0.554 & \textbf{0.237} & \textbf{0.638} & 0.824 & \textbf{0.358} & \textbf{0.771} & 0.364 & \textbf{0.468} & \textbf{0.781} \\
% \midrule
% Lex-Similarity & 0.610 & 0.224 & 0.630 & {0.836} & 0.216 & 0.674 & \textbf{0.728} & 0.394 & 0.736 \\
% Max Entropy & \textbf{0.628} & 0.205 & 0.620 & 0.824 & 0.253 & 0.691 & 0.722 & 0.352 & 0.711 \\
% EigValLaplacian & 0.602 & 0.175 & 0.601 & 0.826 & 0.099 & 0.575 & 0.696 & 0.344 & 0.707 \\
% SAR & 0.612 & 0.227 & 0.632 & 0.830 & 0.276 & 0.709 & 0.718 & 0.384 & 0.731 \\
% Mean Entropy & 0.606 & 0.202 & 0.618 & \textbf{0.840} & 0.319 & 0.742 & 0.716 & 0.365 & 0.719 \\
% \bottomrule
% \end{tabular}
% }

%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{

\begin{tabular}{lccc|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{3}{c|}{NQ} & \multicolumn{3}{c|}{SQUAD} & \multicolumn{3}{c|}{TQA} & \multicolumn{3}{c|}{2Wiki} & \multicolumn{3}{c|}{HotPot} & \multicolumn{3}{c}{Musique} \\
\cmidrule{2-19}
 & Acc & Corr & AUC & Acc & Corr & AUC & Acc & Corr & AUC & Acc & Corr & AUC & Acc & Corr & AUC & Acc & Corr & AUC \\
\midrule
AdaptiveRAG & 0.57 & 0.06 & 0.54 & 0.73 & 0.10 & 0.58 & 0.51 & -0.02 & 0.49 & \textbf{0.72} & \textbf{0.34} & \textbf{0.71} & 0.71 & 0.19 & 0.62 & 0.88 & 0.15 & 0.64 \\
DRAGIN & 0.55 & 0.12 & 0.57 & 0.82 & 0.11 & 0.58 & 0.36 & 0.03 & 0.52 & 0.68 & -0.07 & 0.46 & 0.71 & 0.01 & 0.51 & \underline{0.89} & -0.01 & 0.49 \\
FLARE & 0.59 & 0.16 & 0.59 & 0.54 & 0.11 & 0.58 & 0.58 & 0.12 & 0.57 & 0.51 & 0.20 & 0.62 & 0.42 & 0.06 & 0.54 & 0.59 & 0.01 & 0.51 \\
Rowen\textsubscript{CL} & 0.45 & -0.14 & 0.44 & 0.18 & -0.06 & 0.47 & 0.64 & -0.07 & 0.47 & 0.32 & -0.10 & 0.46 & 0.29 & -0.13 & 0.44 & 0.11 & 0.00 & 0.50 \\
Rowen\textsubscript{CM} & 0.45 & -0.03 & 0.49 & 0.18 & -0.06 & 0.47 & 0.64 & -0.13 & 0.44 & 0.32 & 0.02 & 0.51 & 0.29 & -0.14 & 0.44 & 0.11 & -0.02 & 0.49 \\
Rowen\textsubscript{Hybrid} & 0.45 & -0.12 & 0.44 & 0.17 & -0.07 & 0.46 & 0.63 & -0.13 & 0.43 & 0.32 & -0.04 & 0.48 & 0.29 & -0.17 & 0.41 & 0.11 & -0.01 & 0.49 \\
Seakr & 0.55 & \textbf{0.24} & \textbf{0.64} & 0.82 & \textbf{0.36} & \textbf{0.77} & 0.36 & \textbf{0.47} & \textbf{0.78} & 0.68 & -0.22 & 0.37 & 0.71 & 0.08 & 0.55 & \underline{0.89} & 0.06 & 0.56 \\
\midrule
EigValLaplacian & 0.60 & 0.17 & 0.60 & 0.83 & 0.10 & 0.57 & 0.70 & 0.34 & 0.71 & \underline{0.69} & 0.19 & 0.62 & \textbf{0.73} & 0.27 & 0.67 & \underline{0.89} & 0.12 & 0.62 \\

Lex-Similarity & \underline{0.61} & 0.22 & \underline{0.63} & \textbf{0.84} & 0.22 & 0.67 & \textbf{0.73} & \underline{0.39} & \underline{0.74} & 0.68 & 0.21 & 0.63 & \textbf{0.73} & 0.30 & 0.69 & \textbf{0.90} & 0.08 & 0.59 \\
Max Entropy & \textbf{0.63} & 0.20 & 0.62 & 0.82 & 0.25 & \underline{0.69} & 0.72 & 0.35 & 0.71 & 0.69 & 0.19 & 0.62 & \textbf{0.73} & 0.29 & 0.69 & \underline{0.89} & \textbf{0.18} & \textbf{0.67} \\
Mean Entropy & \underline{0.61} & 0.20 & 0.62 & \textbf{0.84} & \underline{0.32} & \underline{0.74} & 0.72 & 0.36 & 0.72 & 0.68 & \underline{0.28} & \underline{0.68} & \underline{0.72} & \textbf{0.31} & \textbf{0.70} & \textbf{0.90} & 0.15 & 0.64 \\
SAR & \underline{0.61} & \underline{0.23} & \underline{0.63} & \underline{0.83} & 0.28 & 0.71 & 0.72 & 0.38 & 0.73 & \underline{0.69} & 0.23 & 0.65 & \textbf{0.73} & 0.30 & 0.69 & \underline{0.89} & \underline{0.17} & \underline{0.66} \\
\bottomrule
\end{tabular}
}
    \caption{\textbf{Self-knowledge} metrics for adaptive retrieval and uncertainty methods. `Acc' and `AUC' refer to accuracy and ROC-AUC, respectively, for identifying self-knowledge. `Corr' denotes the Spearman correlation with the self-knowledge label. Bold values indicate the highest score,  underlined values represent the second-highest score.}
    \label{tab:main_proxy}
    \vspace{-0.2cm}
\end{table*}



==> tables/main_results.tex <==
% table with baselines, 3 UC (max over classifiers), best UC and Ideal Classifier (Oracle) over datasets
% columns = in-accuracy, retrieval call, llm call (do we need EM and F1 there?)
% +- std bootstrapped over test set

% support by average rank over accuracy, llm, retrieval call figure. either a star figure or smth representative

% somehow rank stability should be shown, either add rank and std in table or add conf intervals to plot, or both
% the main idea is that methods are not stable and might perform sometimes very well and sometimes not

% Artem has also proposed to use normalized performance. Might be a usefull idea for plotting. Normalize over the ideal UC (the Oracle)


% \begin{table*}
%     \centering
%     \begin{tabular}{lccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{{Method}} & \multicolumn{3}{c|}{NQ} & \multicolumn{3}{c|}{SQUAD} & \multicolumn{3}{c}{TQA} \\
%  & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC \\
% \midrule
% AdaptiveRAG & 0.496 & 1.0 & 0.98 & 0.286 & 1.0 & 0.97 & 0.628 & 0.5 & 0.54 \\
% DRAGIN & 0.480 & 4.5 & 2.24 & 0.298 & 4.3 & 2.14 & 0.666 & 4.1 & 2.06 \\
% FLARE & 0.450 & 3.1 & 2.07 & 0.238 & 3.1 & 2.08 & 0.648 & 2.1 & 1.39 \\
% %Rowen\textsubscript{CL} & 0.494 & 29.5 & 7.24 & 0.196 & 29.2 & 7.19 & 0.656 & 28.7 & 7.06 \\
% %Rowen\textsubscript{CM} & 0.494 & 29.5 & 7.27 & 0.196 & 29.2 & 7.20 & 0.656 & 28.7 & 7.12 \\
% Rowen\textsubscript{Hybrid} & 0.494 & 55.0 & 7.27 & 0.196 & 54.3 & 7.15 & 0.656 & 53.4 & 6.93 \\
% Seakr & 0.406 & 14.6 & 1.00 & 0.268 & 14.6 & 1.00 & 0.656 & 14.6 & 1.00 \\
% \midrule
% EigValLaplacian & 0.512 & 1.0 & 0.81 & 0.314 & 1.0 & 1.00 & 0.640 & 1.0 & 0.26 \\
% Lex-Similarity & 0.512 & 1.0 & 0.58 & 0.318 & 1.0 & 0.96 & 0.646 & 1.0 & 0.22 \\
% Max Entropy & 0.506 & 1.0 & 0.73 & 0.312 & 1.0 & 1.00 & 0.650 & 1.0 & 0.22 \\
% %Mean Entropy & 0.498 & 1.0 & 0.88 & 0.314 & 1.0 & 0.95 & 0.650 & 1.0 & 0.30 \\
% %SAR & 0.500 & 1.0 & 0.79 & 0.312 & 1.0 & 1.00 & 0.642 & 1.0 & 0.29 \\
% \midrule
% Best UC & 0.512 & 1.0 & 0.81 & 0.318 & 1.0 & 0.98 & 0.662 & 1.0 & 0.28 \\
% \midrule
% Ideal & 0.608 & 1.0 & 0.55 & 0.360 & 1.0 & 0.82 & 0.736 & 1.0 & 0.36 \\

% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}
%     \centering
%     \begin{tabular}{lccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{{Method}} & \multicolumn{3}{c|}{2Wiki} & \multicolumn{3}{c|}{HotPot} & \multicolumn{3}{c}{Musique} \\
%  & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC \\
% \midrule
% AdaptiveRAG & 0.454 & 2.6 & 2.64 & 0.414 & 2.3 & 2.34 & 0.140 & 3.6 & 3.63 \\
% DRAGIN & 0.456 & 5.8 & 2.92 & 0.430 & 5.1 & 2.56 & 0.134 & 6.3 & 3.15 \\

% FLARE & 0.424 & 3.9 & 2.85 & 0.372 & 5.1 & 4.07 & 0.090 & 4.1 & 3.10 \\
% % Rowen_CL & 0.444 & 32.9 & 7.87 & 0.354 & 31.9 & 7.67 & 0.104 & 42.1 & 9.52 \\
% % Rowen_CM & 0.444 & 32.9 & 7.87 & 0.356 & 31.9 & 7.70 & 0.104 & 42.1 & 9.52 \\
% Rowen\textsubscript{Hybrid} & 0.444 & 61.8 & 7.85 & 0.354 & 59.8 & 7.63 & 0.102 & 80.2 & 9.48 \\
% Seakr & 0.398 & 12.3 & 2.44 & 0.424 & 9.9 & 1.76 & 0.118 & 12.3 & 2.40 \\
% \midrule
% EigValLaplacian & 0.384 & 1.0 & 0.98 & 0.410 & 1.0 & 0.91 & 0.102 & 1.0 & 1.00 \\
% Lex-Similarity & 0.376 & 1.0 & 0.97 & 0.410 & 1.0 & 0.95 & 0.100 & 1.0 & 1.00 \\
% Max Entropy & 0.376 & 1.0 & 0.95 & 0.414 & 1.0 & 0.99 & 0.100 & 1.0 & 1.00 \\
% %Mean Entropy & 0.378 & 1.0 & 0.93 & 0.410 & 1.0 & 0.99 & 0.100 & 1.0 & 1.00 \\
% %SAR & 0.380 & 1.0 & 0.97 & 0.412 & 1.0 & 0.90 & 0.100 & 1.0 & 1.00 \\
% \midrule
% Best UC & 0.384 & 1.0 & 0.98 & 0.414 & 1.0 & 0.99 & 0.104 & 1.0 & 0.99 \\

% \midrule
% Ideal & 0.500 & 1.0 & 0.68 & 0.460 & 1.0 & 0.71 & 0.164 & 1.0 & 0.89 \\

% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[ht!]
    \centering
    \small
    \resizebox{\textwidth}{!}{

    \begin{tabular}{lccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{{Method}} & \multicolumn{3}{c|}{NQ} & \multicolumn{3}{c|}{SQUAD} & \multicolumn{3}{c|}{TQA} & \multicolumn{3}{c|}{2Wiki} & \multicolumn{3}{c|}{HotPot} & \multicolumn{3}{c}{Musique} \\
    \cmidrule{2-19}
     % & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC & InAcc & LMC & RC \\
      & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ & InAcc $\uparrow$ & LMC $\downarrow$ & RC $\downarrow$ \\
    \midrule
    Never RAG & 0.446 & 1.0 & 0.00 & 0.176 & 1.0 & 0.00 & 0.636 & 1.0 & 0.00 & 0.318 & 1.0 & 0.00 & 0.286 & 1.0 & 0.00 & 0.106 & 1.0 & 0.00 \\

    Always RAG & 0.496 & 1.0 & 1.00 & 0.312 & 1.0 & 1.00 & 0.610 & 1.0 & 1.00 & 0.374 & 1.0 & 1.00 & 0.410 & 1.0 & 1.00 & 0.100 & 1.0 & 1.00 \\
    \midrule
    IRCoT & 0.478 & 2.7 & 2.70 & 0.268 & 2.7 & 2.68 & 0.608 & 2.7 & 2.74 & 0.454 & 4.4 & 4.38 & \textbf{0.438} & 3.5 & 3.45 & 0.138 & 4.1 & 4.08 \\


    AdaptiveRAG & 0.496 & 2.0 & 0.98 & 0.286 & 2.0 & 0.97 & 0.628 & 1.5 & 0.54 & 0.454 & 5.2 & 2.64 & 0.414 & 4.6 & 2.34 & \textbf{0.140} & 3.6 & 3.63 \\
    DRAGIN & 0.480 & 4.5 & 2.24 & 0.298 & 4.3 & 2.14 & \textbf{0.666} & 4.1 & 2.06 & \textbf{0.456} & 5.8 & 2.92 & 0.430 & 5.1 & 2.56 & 0.134 & 6.3 & 3.15 \\

    FLARE & 0.450 & 3.1 & 2.07 & 0.238 & 3.1 & 2.08 & 0.648 & 2.1 & 1.39 & 0.424 & 3.9 & 2.85 & 0.372 & 5.1 & 4.07 & 0.090 & 4.1 & 3.10 \\

    Rowen\textsubscript{CL} & 0.494 & 29.5 & 7.24 & 0.196 & 29.2 & 7.19 & 0.656 & 28.7 & 7.06 & 0.444 & 32.9 & 7.87 & 0.354 & 31.9 & 7.67 & 0.104 & 42.1 & 9.52 \\
     Rowen\textsubscript{CM} & 0.494 & 29.5 & 7.27 & 0.196 & 29.2 & 7.20 & 0.656 & 28.7 & 7.12 & 0.444 & 32.9 & 7.87 & 0.356 & 31.9 & 7.70 & 0.104 & 42.1 & 9.52 \\
    Rowen\textsubscript{Hybrid} & 0.494 & 55.0 & 7.27 & 0.196 & 54.3 & 7.15 & 0.656 & 53.4 & 6.93 & 0.444 & 61.8 & 7.85 & 0.354 & 59.8 & 7.63 & 0.102 & 80.2 & 9.48 \\
    
    Seakr & 0.406 & 14.6 & 1.00 & 0.268 & 14.6 & 1.00 & 0.656 & 14.6 & 1.00 & 0.398 & 12.3 & 2.44 & 0.424 & 9.9 & 1.76 & 0.118 & 12.3 & 2.40 \\

    \midrule
    EigValLaplacian & \textbf{0.512} & 1.8 & 0.81 & 0.314 & 2.0 & 1.00 & 0.640 & 1.3 & 0.26 & \textbf{0.384} & 2.0 & 0.98 & 0.410 & 1.9 & 0.91 & \textbf{0.102} & 2.0 & \textbf{0.99} \\

    Lex-Similarity & \textbf{0.512} & 1.6 & \textbf{0.58} & \textbf{0.318} & 2.0 & \textbf{0.96} & 0.646 & 1.2 & 0.22 & 0.376 & 2.0 & 0.97 & 0.410 & 2.0 & 0.95 & 0.100 & 2.0 & 1.00 \\

    Max Entropy & 0.506 & 1.7 & 0.73 & 0.312 & 2.0 & 1.00 & 0.650 & 1.2 & \textbf{0.22} & 0.376 & 2.0 & 0.95 & \textbf{0.414} & 2.0 & 0.99 & 0.100 & 2.0 & 1.00 \\

    Mean Entropy & 0.498 & 1.9 & 0.88 & 0.314 & 2.0 & \textbf{0.95} & 0.650 & 1.3 & 0.30 & 0.378 & 1.9 & \textbf{0.93} & 0.410 & 2.0 & 0.99 & 0.100 & 2.0 & 1.00 \\


    SAR & 0.500 & 1.8 & 0.79 & 0.312 & 2.0 & 1.00 & 0.642 & 1.3 & 0.29 & 0.380 & 2.0 & 0.97 & 0.412 & 1.9 & \textbf{0.90} & 0.100 & 2.0 & 1.00 \\

    \midrule
    Best UE & \textbf{0.512} & 1.8 & 0.81 & \textbf{0.318} & 2.0 & 0.96 & \textbf{0.662} & 1.3 & 0.28 & \textbf{0.384} & 2.0 & 0.98 & \textbf{0.414} & 2.0 & 0.99 & \textbf{0.104} & 2.0 & \textbf{0.99} \\

    \midrule
    Ideal & 0.608 & 1.6 & 0.55 & 0.360 & 1.8 & 0.82 & 0.736 & 1.4 & 0.36 & 0.500 & 1.7 & 0.68 & 0.460 & 1.7 & 0.71 & 0.164 & 1.9 & 0.89 \\

    \bottomrule
    \end{tabular}
    }

    \caption{QA Performance of adaptive retrieval and uncertainty methods. `Best UE' refers to the top-performing uncertainty estimation method for each dataset. `Ideal' represents the performance of a system with an oracle providing ideal predictions for the need to retrieve. `InAcc' denotes In-Accuracy, measuring the QA system's performance. `LMC' indicates the mean number of LM calls per question, and `RC' represents the mean number of retrieval calls per question.}
    \label{tab:main_results}

\end{table*}

==> tables/metrics_corr.tex <==
\begin{table}[th!]
    \centering
    \begin{tabular}{lrrrrrr}
    \toprule
     & InAcc & EM & F1 & Acc & AUC & Corr \\
    \midrule
    InAcc & 1.00 & 0.63 & 0.75 & 0.09 & -0.02 & 0.05 \\
    EM & 0.63 & 1.00 & 0.93 & -0.12 & 0.09 & 0.09 \\
    F1 & 0.75 & 0.93 & 1.00 & -0.06 & 0.08 & 0.09 \\
    Acc & 0.09 & -0.12 & -0.06 & 1.00 & 0.21 & 0.15 \\
    AUC & -0.02 & 0.09 & 0.08 & 0.21 & 1.00 & 0.79 \\
    Corr & 0.05 & 0.09 & 0.09 & 0.15 & 0.79 & 1.00 \\
    \bottomrule
    \end{tabular}
    \caption{Spearman correlations between evaluation metrics normalized across each dataset. The result reveals a low correlation between downstream metrics (InAcc, EM, F1) and self-knowledge metrics (Acc, AUC, Corr). This underscores the importance of conducting a more comprehensive evaluation of self-knowledge of adaptive retrieval systems, rather than relying solely on downstream performance.}
    \label{tab:metric_corr}
\end{table}

==> tables/stat_ood.tex <==
\input{tables/UE_description_part1}\begin{table*}[t]
    \centering
    \begin{tabular}{lccccc}
    \toprule
    Method & EigValLaplacian & Lex-Similarity & Max Entropy & Mean Entropy & SAR \\
    \midrule
    EigValLaplacian & 1.00 & 0.03 & 0.81 & 0.00 & 0.00 \\
    Lex-Similarity & 0.03 & 1.00 & 0.38 & 0.42 & 0.95 \\
    Max Entropy & 0.81 & 0.38 & 1.00 & 0.00 & 0.08 \\
    Mean Entropy & 0.00 & 0.42 & 0.00 & 1.00 & 0.86 \\
    SAR & 0.00 & 0.95 & 0.08 & 0.86 & 1.00 \\
    \bottomrule
    \end{tabular}
    \caption{In-Accuracy P-Value, Friedman Test Results:
Test Statistic: 29.580
P-value: 0.00001}
    \label{tab:qa_ood_test}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{lccccc}
    \toprule
    Method & EigValLaplacian & Lex-Similarity & Max Entropy & Mean Entropy & SAR \\
    \midrule
    EigValLaplacian & 1.00 & 0.00 & 0.08 & 0.00 & 0.05 \\
    Lex-Similarity & 0.00 & 1.00 & 0.81 & 0.94 & 0.88 \\
    Max Entropy & 0.08 & 0.81 & 1.00 & 0.33 & 1.00 \\
    Mean Entropy & 0.00 & 0.94 & 0.33 & 1.00 & 0.42 \\
    SAR & 0.05 & 0.88 & 1.00 & 0.42 & 1.00 \\
    \bottomrule
    \end{tabular}
    \caption{Accuracy P-Value, Friedman Test Results:
Test Statistic: 22.847
P-value: 0.00014}
    \label{tab:self_knowledge_ood_test}
\end{table*}

% Friedman Test Results:
%Test Statistic: 2.359
%P-value: 0.67005


==> tables/transfer_top1UC_table.tex <==
% 6x6 table with showing top-1 UC transfer ability
